Adversarial Learning of Robust and Safe Controllers for Cyber-Physical Systems

We introduce a novel learning-based approach to synthesize safe and robust controllers for autonomous Cyber-Physical Systems and, at the same time, to generate challenging tests. This procedure combines formal methods for model verification with Generative Adversarial Networks. The method learns two Neural Networks: the first one aims at generating troubling scenarios for the controller, while the second one aims at enforcing the safety constraints. We test the proposed method on a variety of case studies.

==> sections/Methodology.tex <==
\section{Methodology}



\paragraph*{Agent-Environment Model.}
Due to coexistence of continuous and discrete components, CPSs are typically represented as hybrid models: the continuous part is represented by differential equations that describe the behaviour of the plant; the discrete part, instead, identifies the possible states of the controller. 
We decompose our model in two interacting parts: the \emph{agent} $a$ and the \emph{environment} $e$. Both of them are able to observe at least part of the whole state space $\mathcal{S}$, i.e. they are aware of some observable states $\mathcal{O}\subset\mathcal{S}$.
 %$\dim\mathcal{O}=m\le \dim\mathcal{S}=n$.
By distinguishing between the observable states of the agent $\mathcal{O}_a\subseteq \mathcal{O}$ and of the environment $\mathcal{O}_b\subseteq \mathcal{O}$, we are able to force uneven levels of knowledge between them.

Let $\mathcal{U}_a$ and $\mathcal{U}_e$ be the spaces of all possible actions for the two components. We discretize the evolution of the system as a discrete-time system with step $\Delta t$, which evolves according to a function $\psi: \mathcal{S} \times \mathcal{U}_a \times \mathcal{U}_e \times \mathbb{R} \longrightarrow \mathcal{S}$.
By taking control actions at fixed time intervals of length $\Delta t$, we obtain a discrete evolution of the form  $ s_{i+1} = s_i + \psi(s_i, u_a^i, u_e^i, t_i)$, where $t_i := t_0 + i\cdot\Delta t$, $u^i := u(t_i)$ and $s_i := s(t_i)$.  Therefore, we are able to simulate the entire evolution of the system over a time horizon $H$ via $\psi$ and to obtain a complete trajectory $\xi=s_0 \dots s_{H-1}$ in the state space.


\paragraph*{Weighted robustness.}
The safety requirement is expressed as a Signal Temporal Logic formula $\Phi$ over a finite time horizon $k$.
We are leveraging the notion of robustness in quantitative semantics to measure the satisfiability of the STL property and to determine how safe the system is in a given configuration.
We denote robustness as a function $R_{\Phi}: \mathcal{S}^k \rightarrow \mathbb{R}$, measuring the maximum shift that can be applied to a given trajectory  $\xi$ of length $k$ without changing the truth value of $\Phi$. %\luca{Da qualche parte va detto che le formule che usiamo sono time bounded e che k is larger that the temporal horizon of the formula. In footnote: temporal horizon is defined recursively as bla bla bla.}
It is straightforward to use this measure as the objective function in our minmax game. 

%\fc{Tento di riformulare il seguente paragrafo in modo più chiaro.}
%In the case of multiple safety requirements the objective function is the weighted sum of the resulting robustness values and the choice of their weights is case-specific. This formulation, solves the problem of different orders of magnitude in the physical components of the hybrid system, causing an unbalanced optimization in terms of robustness. A similar approach is proposed by \cite{li_belta}, where the robustness values from the individual predicates are normalized before being combined together.

In case of multiple safety requirements, we define a STL formula for each property and compute the relative robustness value. As a matter of fact, the order of magnitude of the robustness values depends on the order of magnitude of the CPS variables involved. Therefore, a single STL formula that combines all the safety requirements may produce an unbalanced objective function, skewed towards some components that are not necessarily the more safety-critical. To overcome this problem we define the objective function as a weighted sum of the robustness values resulting from each requirement. 
\fc{Let $\Phi=\{\Phi_1,\dots, \Phi_m\}$ denote a set of $m$ safety requirements, the weighted robustness $R_{\Phi}$ is defined as:
\begin{equation*}
R_{\Phi}(\cdot) := \frac{1}{W}\sum_{i=1}^m w_i\cdot R_{\Phi_i}(\cdot),    
\end{equation*}
where $W= \sum_{i=1}^m w_i$.}
The weights $w_1,\dots, w_m$ become important hyper-parameters and their tuning will be case-specific.  This formulation is typically used in multi-objective optimization scenarios ~\citep{li_belta}.
 %\gc{molto meglio!}

\paragraph*{Attacker-Defender architecture.} 
The proposed framework builds on GAN architectural design, in which two NNs compete in a minmax game to reach opposite goals.
One network, denoted by $A$, represents the \textit{attacker}, while the other, denoted by $D$, represents the \textit{defender}. The aim of the former is to generate environment configurations in which the defender is not able to act safely, whereas, the latter tries to keep the CPS as safe as possible. 
In practice, the defender $D$ can be interpreted as a controller for the agent.



The evolution $\xi$ starts from a given state of the system $s_0$ at time $t_0$ and it is obtained by 
evaluating $\psi$ at time steps $t_i\in\{t_0,\dots, t_{H-1}\}$ %t_i=t_0,\dots, t_{H-1}$
over two sequences of actions $\textbf{u}_a = (u_a^0, \dots, u_a^{H-1} )$ and $ \textbf{u}_e = (u_e^0, \dots, u_e^{H-1} )$.
Let $\theta_A$ be the weights of the attacker's network $A$ and $\theta_D$ the weights of the defender's network $D$. At each timestep, the attacking network, 
\begin{align*}
A: \Theta_A \times \mathcal{O}_e \times \mathcal{Z} &\longrightarrow \mathcal{U}_e \\
(\theta_A, \textbf{o}_e, \textbf{z}) & \longmapsto u_e,
\end{align*} 
receives the current observable state of the environment $\mathbf{o}_e$ and outputs the coefficients $u_e$, defining the adversarial environmental components. $A$ is the generative part of the underlying GAN model and the noise term $\mathbf{z}\in \mathcal{Z}$ allows it to learn the distribution of the observed states $\textbf{o}_e$.
Similarly, the defender network,
\begin{align*}
D: \Theta_D \times \mathcal{O}_a &\longrightarrow \mathcal{U}_a \\
(\theta_D, \textbf{o}_a) & \longmapsto u_a,
\end{align*}
reads the current observable state of the agent $\mathbf{o}_a$ and produces the control action $u_a$.



\paragraph*{Optimization strategy.}

The objective function \fc{$\mathscr{L}$}\gc{$\mathcal{J}$?} in our minmax problem, 
\begin{equation}
\min_{\textbf{u}_e}\max_{\textbf{u}_a} \mathscr{L}(s_0, \textbf{u}_a, \textbf{u}_e),
\end{equation}
\fc{la L indica tipicamente la loss, mentre noi usiamo una sorta di reward. Proporrei di usare o -R come loss o invece che L userei la lettera j più comune in caso di objective functions generiche.}
is the cumulative sum of the robustness values computed at each timestep during the generation of the whole trajectory $\xi$ on the sub-trajectory $\xi[t-k,t]$ available at timestep $t$, i.e.
$$
\mathscr{L}(s_0, \textbf{u}_a, \textbf{u}_e) := 
\mathlarger\sum_{t=k}^{H-1}R_{\Phi}(\xi[t-k,t]).
$$

In particular, requirements will be defined in terms of the time-bounded operator $\mathsf{historically}_k$, indicating that the given property has to hold everywhere in the last $k$ timesteps $[t-k,t]$ for an input trajectory $\xi_t$ of length $t$. \fc{Questa frase non mi convince, cerco di riformularla ASAP.}

For convenience, we introduce 
\begin{align*}
F_t: \mathcal{S} \times \Theta_D \times \Theta_A &\longrightarrow \mathcal{S}^t
\\
(s_0, \theta_D, \theta_A) &\longmapsto \xi,
\end{align*}
\fc{qui $\xi$ non infdica niente di chiaro, userei forse $s_0 s_1 \dots, s_{t-1}$ come notazione. Inoltre se usiamo $\psi$ qui userei $\Psi$ non $F$.} 
which iteratively applies $\psi$ for each pair of actions 
\begin{align*}
u_a^j &= D(\theta_D, \textbf{o}_a^j)\\
u_e^j &= A(\theta_A, \textbf{o}_e^j, \textbf{z}), 
\end{align*}
where $j\in [0,t-1]$ indexes the simulation interval.

The formalism introduced by the two policy networks transfers the
problem of finding the best sequences of actions, $\textbf{u}_a$ and $\textbf{u}_e$, to that of finding the best networks' parameters, $\theta_D$ and $\theta_A$.
This leads to the objective 
$$
\mathcal{L}(\theta_A, \theta_D) =
\mathlarger\sum_{t=k}^{H-1}
R_{\Phi}[F_t(s_0, \theta_D, \theta_A)]
$$
\fc{se ho capito bene, la $t$ in $F_t$ indica la lunghezza della traiettoria e $s_0$ l'istante iniziale del meccanismo forward. Inoltre la loss continua a dipendere da $s_0$ giusto? Quindi sarebbe 
\begin{equation*}
    \mathcal{L}(s_0,\theta_A, \theta_D) =
\mathlarger\sum_{t=k}^{H-1}
R_{\Phi}[F_k(s_{t-k}, \theta_D, \theta_A)]
\end{equation*}
}
and the minmax game $ {\min}_{\theta_A} \; {\max}_{\theta_D} \; \mathcal{L}(\theta_A, \theta_D)$ is now directly expressed in terms of the training parameters.
In such setting, the defender aims at generating safe actions by tuning its weights in favour of a loss minimization (i.e. robustness maximization). The attacker, instead, aims at generating troubling scenarios for the opponent by maximizing the loss (i.e., minimizing the robustness).\fc{parlare così di loss confonde, come detto nella nota prima}

In the testing phase, the safety requirement is checked on the whole trajectory $\xi_H$, i.e. we simply use the STL operator $\mathsf{globally}$.\fc{non chiaro cosa intendi qui}



